Non-parametric estimation of net survival under dependence between death causes

Relative survival methodology deals with a competing risks survival model where the cause of death is unknown. This lack of information occurs regularly in population-based cancer studies. Non-parametric estimation of the net survival is possible through the Pohar Perme estimator. Derived similarly to Kaplan-Meier, it nevertheless relies on an untestable independence assumption. We propose here to relax this assumption and provide a generalized non-parametric estimator that works for other dependence structures, by leveraging the underlying stochastic processes and martingales. We formally derive asymptotics of this estimator, providing variance estimation and log-rank-type tests. Our approach provides a new perspective on the Pohar Perme estimator and the acceptability of the underlying independence assumption. We highlight the impact of this dependence structure assumption on simulation studies, and illustrate them through an application on registry data relative to colorectal cancer, before discussing potential extensions of our methodology.

==> paper-pratendExtraMaterial.tex <==


\begin {figure}[H] \centering \includegraphics [width=\textwidth ]{assets/simus/featherplot2.png} \caption {\label {fig:simus/featherplot2} Each graph shows (in blue) the $N=1000$ survival curves $t \to \hat {S}_E^{(1)}(t),...,t \to \hat {S}_E^{(N)}(t)$ estimated under $\HC $ on resamples simulated using $\mathcal C_0$. Abscissa represents time $t$ in years. The true survival curve $S_E(t)$ of $E \sim \texttt {Exponential}(\mu =10)$ is depicted in orange as a target reference. The true dependence structure $\mathcal C_0$ varies with the line, while the dependence structure assumed by the estimators $\mathcal C$ varies across columns: plots on the diagonal thus correspond to well-specified cases $\mathcal C = \mathcal C_0$.} \end {figure}

\begin {table}[H] \centering \footnotesize \caption {\label {tab:simus/rez5} Observed bias, root-mean-square error and empirical coverage rate over the $N=1000$ simulations at time $t=5$. Lines represent the true copula $\mathcal C_0$ and columns the hypothesized one $\mathcal C$. Smaller bias and root-mean-square errors are better, while empirical coverage rates closer to $95\%$ are better.} \input {assets/simus/rez5.tex} \end {table} \begin {table}[H] \centering \footnotesize \caption {\label {tab:simus/rez10} Observed bias, root-mean-square error and empirical coverage rate over the $N=1000$ simulations at time $t=10$. Lines represent the true copula $\mathcal C_0$ and columns the hypothesized one $\mathcal C$. Smaller bias and root-mean-square errors are better, while empirical coverage rates closer to $95\%$ are better.} \input {assets/simus/rez10.tex} \end {table}

\begin {table}[H] \centering \footnotesize \caption {\label {tab:simus/test1/tst5} (Scenario 1) Rejection rate at $\alpha =5\%, T=5$, with their (asymptotically Gaussian) confidence intervals. Lines represent the true copula $\mathcal C_0$ and columns the hypothesized one $\mathcal C$, in each of the alternatives $H_0,H_1$ and $H_2$.} \input {assets/simus/test1/tst5.tex} \end {table} \begin {table}[H] \centering \footnotesize \caption {\label {tab:simus/test1/tst10} (Scenario 1) Rejection rate at $\alpha =5\%, T=10$, with their (asymptotically Gaussian) confidence intervals. Lines represent the true copula $\mathcal C_0$ and columns the hypothesized one $\mathcal C$, in each of the alternatives $H_0,H_1$ and $H_2$.} \input {assets/simus/test1/tst10.tex} \end {table}

\begin {table}[H] \centering \footnotesize \caption {\label {tab:simus/test2/tst5} (Scenario 2) Rejection rate at $\alpha =5\%, T =5$, with their (asymptotically Gaussian) confidence intervals. Lines represent the true copula $\mathcal C_0$ and columns the hypothesized one $\mathcal C$, in each of the alternatives $H_0,H_1$ and $H_2$.} \input {assets/simus/test2/tst5.tex} \end {table} \begin {table}[H] \centering \footnotesize \caption {\label {tab:simus/test2/tst10} (Scenario 2) Rejection rate at $\alpha =5\%, T=10$, with their (asymptotically Gaussian) confidence intervals. Lines represent the true copula $\mathcal C_0$ and columns the hypothesized one $\mathcal C$, in each of the alternatives $H_0,H_1$ and $H_2$.} \input {assets/simus/test2/tst10.tex} \end {table}

\begin {figure}[H] \centering \includegraphics [width=\textwidth ]{assets/example/short_paper_graph_var.png} \caption {\label {fig:example/short_paper_graph_var} Estimated standard errors $t \to \hat {\sigma }_E(t)$ on the left and right tumor locations, for various hypothesized copulas $\mathcal C$. For both the Frank and Clayton copula, $\tau =0$ represents the Pohar Perme variance.} \end {figure}


==> paper-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}We prove items in the exposing order. Remark first that$\P {P=E=t}=0$ by absolute continuity, and then: \begin {align*} \E {\partial N(t)}{E,C} &= \P {E \wedge P = t, t \le C}{E,C}\\ &= \P {P \ge t, E = t, t \le C}{E,C} + \P {t \le E, P = t, t \le C}{E,C}\\ &= \P {P \ge t}{E = t}\I {E = t, E \le C} + \P {P = t}{E \ge t}\I {E \ge t, C \ge t}\\ &= a(t) \partial N_E(t) + b(t) Y_E(t). \end {align*} Moreover, \begin {align*} \E {Y(t)}{E,C} &= \P {E\wedge P \ge t, C \ge t}{E,C}\\ &= \P {P \ge E \ge t, C \ge t}{E,C} + \P {E \ge P \ge t, C \ge t}{E,C}\\ &= \P {P \ge E}{E \ge t} Y_E(t) + \P {E \ge P \ge t}{E \ge t}Y_E(t)\\ &= \P {P \ge t}{E \ge t} Y_E(t)\\ &= c(t) Y_E(t). \end {align*} \Cref {lem:tech:1,lem:tech:Y} follow from inverting this system of two equations to extract $(\partial N_E(t), Y_E(t))$. To prove \cref {lem:tech:2}, recall that $\partial \Lambda _X(t) = \frac {\P {X = t}}{\P {X \ge t}}$ for $X \in {E,O}$, and expand $a(t),b(t),c(t)$: \begin {align*} \frac {c(t)}{a(t)}\left (\partial \Lambda _O(t) - \frac {b(t)}{c(t)}\right ) &= \frac {\P {P \ge t}{E \ge t}}{\P {P \ge t}{E = t}}\left (\frac {\P {O = t}}{\P {O \ge t}} - \frac {\P {P = t}{E \ge t}}{\P {P \ge t}{E \ge t}}\right )\\ &= \frac {\P {E = t}}{\P {E \ge t}}\frac {\P {P \ge t , E \ge t}}{\P {P \ge t , E = t}}\left (\frac {\P {O = t}}{\P {O \ge t}} - \frac {\P {P = t , E \ge t}}{\P {P \ge t , E \ge t}}\right )\\ &= \partial \Lambda _E(t)\frac {\P {O \ge t}}{\P {P \ge t , E = t}}\left (\frac {\P {O = t} - \P {P = t , E \ge t}}{\P {O \ge t}}\right )\\ &= \partial \Lambda _E(t)\frac {\P {O = t} - \P {P = t , E \ge t}}{\P {P \ge t , E = t}}\\ &= \partial \Lambda _E(t). \end {align*} \par To prove \cref {lem:tech:3}, using \cref {lem:tech:1,lem:tech:Y,lem:tech:2}, consider first that \begin {align*} \Etm {\partial N_E(t)} &= \Etm {\frac {1}{a(t)}\E {\partial N(t)}{E,C} - \frac {b(t)}{a(t)c(t)} \E {Y(t)}{E,C}}\\ &= \E {\frac {1}{a(t)}\Etm {\partial N(t)} - \frac {b(t)}{a(t)c(t)} Y(t)}{E,C}\\ &= \E {\frac {Y(t)}{a(t)}\left (\partial \Lambda _O(t) - \frac {b(t)}{c(t)}\right )}{E,C}\\ &= \E {Y_E(t) \partial \Lambda _E(t)}{E,C}\\ &= Y_E(t) \partial \Lambda _E(t). \end {align*} Thus, \begin {align*} \partial M_E(t) &= \partial N_E(t) - Y_E(t) \partial \Lambda _E(t)\\ &= \E {\frac {\partial N(t)}{a(t)} - \frac {b(t) Y(t)}{a(t)c(t)} - \frac {Y(t)}{c(t)}\frac {c(t)}{a(t)}\left (\partial \Lambda _O(t) - \frac {b(t)}{c(t)}\right )}{E,C}\\ &= \E {\frac {\partial N(t)}{a(t)} - \frac {Y(t)\partial \Lambda _O(t)}{a(t)}}{E,C}\\ &= \E {\frac {\partial M(t)}{a(t)}}{E,C}. \end {align*} So that $M_E(t) = \E {\int _0^t \frac {\partial M(s)}{a(s)}}{E,C}$ as wanted. Since the function $a$ is predictable, $M_E$ is a martingale and the decomposition is unique.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Let us denote $\forall i \in 1,...,n$: \begin {align*} \partial \tld {M}_{E}(t) &= \frac {\partial M(t)}{a(t)}\\ \partial \tld {M}_{E,i} &= \frac {\partial M_i(t)}{a_i(t)}\\ \partial \Xi (t) &= \frac {\sum _{i=1}^n \partial \tld {M}_{E,i}(t)}{\sum _{i=1}^n \tld {Y}_{E,i}(t)}. \end {align*} We will in fact prove that both $\tld {M}_{E,i}$ and $\Xi $ are local square integrable martingales, and that we have the two following Doob-Meyer decompositions: \begin {itemize} \item $\forall i,$ $\partial \tld {N}_{E,i}(t) = \partial \tld {M}_{E,i}(t) + \tld {Y}_{E,i}(t) \partial \Lambda _E(t),$ \item $\tld {\Lambda }_E(t) = \Lambda _E(t) + \Xi (t).$ \end {itemize} \par Recall first that, for all $i \in 1,...,n$, $$\partial \tld {N}_{E,i}(t) = \frac {1}{a_i(t)} \partial N_i(t) - \frac {b_i(t)}{a_i(t)c_i(t)} Y_i(t).$$ Since $\Etm {\partial N_i(t)} = Y_i(t)\partial \Lambda _{O_i}(t)$, we have by \cref {lem:tech:2} in \cref {lem:tech} that: \begin {align*} \Etm {\partial \tld {N}_{E,i}(t)} &= \frac {1}{a_i(t)} Y_i(t)\partial \Lambda _{O_i}(t) - \frac {b_i(t)}{a_i(t)c_i(t)} Y_i(t)\\ &= \frac {Y_i(t)}{a_i(t)}\left (\partial \Lambda _{O_i}(t) - \frac {b_i(t)}{c_i(t)}\right )\\ &= \frac {Y_i(t)}{c_i(t)}\partial \Lambda _{E_i}(t)\\ &= \tld {Y}_{E,i}(t) \partial \Lambda _E(t). \end {align*} Subtracting the two gives $\partial \tld {M}_{E,i}(t) = \frac {\partial M_i(t)}{a_i(t)}$ as required, and since $ \tld {M}_{E,i}(t)$ is a local square integrable martingale, this decomposition is unique. \par Then, since $a_i(t),b_i(t),c_i(t)$ are constants and since the processes $Y_i$ are $\Ft $-predictables, we have that \begin {align*} \Etm {\partial \tld {\Lambda }_E(t)} &= \Etm {\frac {\sum _{i=1}^n \partial \tld {N}_{E,i}(t)}{\sum _{i=1}^n \tld {Y}_{E,i}(t)}}\\ &=\frac {\sum _{i=1}^n \Etm {\partial \tld {N}_{E,i}(t)}}{\sum _{i=1}^n \tld {Y}_{E,i}(t)}\\ &=\frac {\sum _{i=1}^n \tld {Y}_{E,i}(t) \partial \Lambda _E(t)}{\sum _{i=1}^n \tld {Y}_{E,i}(t)}\\ &= \partial \Lambda _E(t) \end {align*} Subtracting, we obtain the required expression for $\partial \Xi (t)$ as follows: $$\partial \Xi (t) = \partial \tld {\Lambda }_E(t) - \partial \Lambda _E(t) = \frac {\sum _{i=1}^n \frac {1}{a_i(t)}\partial M_i(t)}{\sum _{i=1}^n \frac {Y_i(t)}{c_i(t)}}.$$ Since $Y_i$ is predictable, again, $\Xi $ is a local square integrable martingale and this decomposition is unique.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}From \cite [formula (2.47) and (2.49) p. 56]{aalenSurvivalEventHistory2008}, denoting $\left [\Xi \right ]$ denote the optional processes of $\Xi $, \cref {lem:DMtldlambda} implies that $$\V {\tld {\Lambda }_E(t)} = \E {\left [\Xi \right ](t)}.$$ Due to orthogonality of martingales $M_1,...,M_n$, and since $\forall i$, $$\frac {\frac {1}{a_i(s)}}{\sum _{i=1}^n \frac {Y_i(s)}{c_i(s)}}$$ are predictable processes, we complete the argument by: \begin {align*} \partial \left [\Xi \right ](t) &= \partial \left [\int _{0}^t \frac {\sum _{i=1}^n \frac {1}{a_i(s)}\partial M_i(s)}{\sum _{i=1}^n \frac {Y_i(s)}{c_i(s)}}\right ](t)\\ &= \partial \left [\sum _{i=1}^n \int _{0}^t \frac {\frac {1}{a_i(s)}}{\sum _{i=1}^n \frac {Y_i(s)}{c_i(s)}} \partial M_i(s)\right ](t)\\ &= \partial \sum _{i=1}^n \int _{0}^t \left (\frac {\frac {1}{a_i(s)}}{\sum _{i=1}^n \frac {Y_i(s)}{c_i(s)}}\right )^2 \partial N_i(s)\\ &= \frac {\sum _{i=1}^n \frac {1}{a_i(t)^2}\partial N_i(t)}{\left (\sum _{i=1}^n \frac {Y_i(t)}{c_i(t)}\right )^2}. \end {align*}\end{proof}

\begin{restatable}[Properties of $\bm R, \bm Z$ and $\bm \Gamma $]{lemma}{prAtEndRestatev}\label{thm:prAtEndv}\label {lem:test} Let $T < \infty $. Under $\left (H_0\right )$, assuming that there exists an $\epsilon > 0:\;a_i(t) > \epsilon ,c_i(t)>\epsilon $ over $t \in [0,T]$, the following points hold over $t \in [0,T]$, \begin {enumerate}[(i)] \item \label {itm:Z_centered_lsim} $\bm Z$ is a centered local square integrable martingale \item \label {itm:Cov_Z} $\mathrm {Cov}(\bm Z(t)) = \E {\bm \Gamma (t)}$ \item \label {itm:cv_Gamma} $n^{-1} \bm \Gamma (t) \xrightarrow [n \to \infty ]{\mathbb P} \bm V(t)$, $\bm V$ is deterministic, and both $\bm \Gamma (t)$ and $\bm V(t)$ are semi-definite positives. \item \label {itm:cv_Z} $n^{-\frac {1}{2}}\bm Z(t) \xrightarrow [n\to \infty ]{\mathcal D} \N {0,\bm V(t)}$ \item \label {itm:rank_V} $\mathrm {Ker}(\bm V(t)) = \mathrm {Vect}(\bm 1)$ \end {enumerate}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Consider throughout the proof that $\left (H_0\right )$ holds, and recall definitions of vectors $\bm R(t),\bm Z(t)$, the matrix $\bm \Gamma (t)$ and the test statistic $\tld {\chi }(T)$: \begin {align*} R_g(t) &= \frac {\tld {Y}_{E,g}(t)}{\tld {Y}_{E,\bigcdot }(t)}\\ Z_{g}(t) &= \tld {N}_{E,g}(t) - \int _{0}^t R_g(s) \partial \tld {N}_{E,\bigcdot }(s)\\ \Gamma _{g,h}(t) &= \sum _{\ell \in G} \int _{0}^t \left (\delta _{\ell ,g} - R_g(s)\right )\left (\delta _{\ell ,h} - R_h(s)\right ) \sum _{i \in \ell } \frac {\partial N_i(s)}{a_i(s)^2}.\\ \tld {\chi }(T) &= \bm Z(T)'\bm \Gamma (T)^{-1} \bm Z(T) \end {align*} Let us prove points in their exposing order. \par \emph {Proof of \cref {itm:Z_centered_lsim}:} From \cref {lem:DMtldlambda}, we have, $\forall g \in G \cup \{\bigcdot \}$: $$\partial \tld {N}_{E,g}(t) = \partial \tld {M}_{E,g}(t) + \tld {Y}_{E,g}(t) \partial \Lambda _{E}(t).$$ Thus: \begin {align} \partial Z_{g}(t) &= \partial \tld {N}_{E,g}(t) - R_g(t)\partial \tld {N}_{E,\bigcdot }(t)\nonumber \\ &= \partial \tld {M}_{E,g}(t) + \tld {Y}_{E,g}(t) \partial \Lambda _E(t) - R_g(t) \left (\partial \tld {M}_{E,\bigcdot }(t) + \tld {Y}_{E,\bigcdot }(t) \partial \Lambda _E(t)\right )\nonumber \\ &= \left (\partial \tld {M}_{E,g}(t) - R_g(t)\partial \tld {M}_{E,\bigcdot }(t)\right ) + \left (\tld {Y}_{E,g}(t) \partial \Lambda _E(t) - R_g(t)\tld {Y}_{E,\bigcdot }(t) \partial \Lambda _E(t) \right )\nonumber \\ &= \sum _{\ell \in G} \left (\delta _{g,\ell } - R_g(t)\right )\partial \tld {M}_{E,\ell }(t) + \tld {Y}_{E,g}(t) \left (\partial \Lambda _E(t) - \partial \Lambda _E(t)\right )\nonumber \\ &= \sum _{\ell \in G} \left (\delta _{g,\ell } - R_g(t)\right ) \partial \tld {M}_{E,\ell }(t)\label {eq:Z} \end {align} \par From now on, we denote $$H_{g,\ell }(t) = \delta _{g,\ell } - R_g(t).$$ \par Since $\left (\tld {M}_{E,g}\right )_{g\in G}$ are uncorrelated local square integrable martingales, and $\left (H_{g,\ell }\right )_{g,\ell \in G}$ are predictable processes, $Z_g$ clearly are centered local square integrable martingales themselves. \par \emph {Proof of \cref {itm:Cov_Z}:} We want to show that $\mathrm {Cov}(\bm Z(t)) = \E {\bm \Gamma (t)}$. For that, it would suffice to show that $\forall g,h\in G,\; \Gamma _{g,h}(t) = \left [Z_g,Z_h\right ](t)$, so we now compute $\left [Z_g,Z_h\right ](t)$. \par Since $\left (H_{g,\ell }\right )_{g,\ell \in G}$ are predictable processes and $\left (\tld {M}_{E,g}\right )_{g\in G}$ are uncorrelated local square integrable martingales, \begin {align*} \partial \left [Z_g,Z_h\right ](t) &= \sum _{\ell \in G} H_{g,\ell }(t) H_{h,\ell }(t) \partial \left [ \tld {M}_{E,\ell }\right ](t)\\ &= \sum _{\ell \in G} H_{g,\ell }(t) H_{h,\ell }(t) \sum _{i \in \ell } \frac {\partial \left [ M_i\right ](t)}{a_i(t)^2} \\ &= \sum _{\ell \in G} H_{g,\ell }(t) H_{h,\ell }(t) \sum _{i \in \ell } \frac {\partial N_i(t)}{a_i(t)^2}\\ &= \partial \Gamma _{g,h}(t). \end {align*} \par \emph {Proof of \cref {itm:cv_Gamma}:} We want to prove that, $\forall g,h \in G$, $$\frac {\Gamma _{g,h}(t)}{n} \xrightarrow [n \to \infty ]{\mathbb P} V_{g,h}(t).$$ Recall that we just showed that $$\Gamma _{g,h}(t) = \sum _{\ell \in G} \int _{0}^t H_{g,\ell }(s) H_{h,\ell }(s) \sum _{i \in \ell } \frac {\partial N_i(s)}{a_i(s)^2}.$$ \par Remember that our patients $(E_i,P_i,\bm X_i)$ are $i.i.d$, and assume (without loss of generality) that their group assignment are included in (or driven by) their covariates $\bm X$. Formally, consider that $G$ is a partition of the covariates support $\mathrm {Supp}(\bm X)$, and introduce $\forall \bm x \in \mathrm {Supp}(\bm X)$ the following notations to highlight this: \begin {align*} a_{\bm x}(s) &= \P {P \ge s}{E = s, \bm X = \bm x}\\ b_{\bm x}(s) &= \P {P = s}{E \ge s, \bm X = \bm x}\\ c_{\bm x}(s) &= \P {P \ge s}{E \ge s, \bm X = \bm x}\\ N_{\bm x}(s) &= \I {O \le s, X \ge s \;|\; \bm X = \bm x} \end {align*} \par \par Let us first study the convergence of $R_g(t) = \frac {\tld {Y}_{E,g}(t)}{\tld {Y}_{E,\bigcdot }(t)}$. Note that : \begin {align*} \Etm {\tld {Y}_{E,g}(t)} &= \frac {1}{n}\sum _{i=1}^n \Etm {\tld {Y}_{E,i}(t) \I {\bm X_i \in g}}\\ &= \frac {1}{n}\sum _{i=1}^n Y_{E,i}(t) \I {\bm X_i \in g}\\ &= \frac {1}{n}\sum _{i=1}^n \I {E_i \ge t, C_i \ge t, \bm X_i \in g}\\ &\xrightarrow [n \to \infty ]{\mathbb P} \P {E \ge t, C\ge t, \bm X \in g}, \end {align*} and, likewise, $\Etm {\tld {Y}_{E,\bigcdot }(t)} \xrightarrow [n \to \infty ]{\mathbb P} \P {E \ge t, C\ge t}$. \par \par \par Furthermore, \begin {align*} \V {\tld {Y}_{E,i}(t)} &= \V {\frac {Y_i(t)}{c_i(t)}}\\ &= \frac {1}{c_i(t)^2} \V {Y_i(t)}\\ &\le \frac {1}{c_i(t)^2} \end {align*} where the bounding is drastic but enough for our purposes. Indeed, we assumed that $c_{i}(t) \ge \epsilon $ over $t \in [0,T]$. We therefore have (by squeezing): $$\V {\tld {Y}_{E,\bigcdot }(t)}\xrightarrow [n \to \infty ]{\mathbb P} 0,$$ and similarly $\forall g \in G$, $$\V {\tld {Y}_{E,g}(t)}\xrightarrow [n \to \infty ]{\mathbb P} 0.$$ Hence: \begin {align*} R_g(t) \xrightarrow [n \to \infty ]{\mathbb P} \frac {\P {E \ge t, C\ge t, \bm X \in g}}{\P {E \ge t, C\ge t}} = \P {\bm X \in g}, \end {align*} where the last equality holds since censorship is independent and because we work under $\left (H_0\right )$. \par Finally, under $\left (H_0\right )$, $$H_{g,\{i\}}(s) = \I {\bm X_i \in g} - R_g(s) \xrightarrow [n \to \infty ]{\mathbb P} \I {\bm X_i \in g} - \P {\bm X \in g},$$ \par Denote now $$\Omega _{g,h}(\bm X) = \left (\I {\bm X \in g} - \P {\bm X \in g}\right )\left (\I {\bm X \in h} - \P {\bm X \in h}\right ).$$ \par Since $\left \lvert H_{g,\{i\}}(s) \right \rvert \le 1$, the dominated convergence theorem applies, and we have \begin {align*} \lim _{n \to \infty } \int _{0}^t H_{g,\{i\}}(s) H_{h,\{i\}}(s) \frac {\partial N_i(s)}{a_i(s)^2} &= \int _{0}^t \Omega _{g,h}(\bm X_i) \frac {\partial N_i(s)}{a_i(s)^2}\\ \end {align*} \par Thus, \begin {align*} \lim _{n \to \infty } \frac {\Gamma _{g,h}(t)}{n} &= \lim _{n \to \infty } \frac {1}{n} \sum _{\ell \in G} \int _{0}^t H_{g,\ell }(s) H_{h,\ell }(s) \sum _{i \in \ell } \frac {\partial N_i(s)}{a_i(s)^2}\\ &= \lim _{n \to \infty } \frac {1}{n} \sum _{i=1}^{n} \int _{0}^t H_{g,\{i\}}(s) H_{h,\{i\}}(s) \frac {\partial N_i(s)}{a_i(s)^2}\\ &= \E {\int _{0}^t \Omega _{g,h}(\bm X) \frac {\partial N_{\bm X}(s)}{a_{\bm X}(s)^2}}\\ &= \E {\Omega _{g,h}(\bm X) \int _{0}^t \frac {\partial N_{\bm X}(s)}{a_{\bm X}(s)^2}}. \end {align*} \par We cannot unfortunately give a simpler expression for this limit, but we can however prove that it exists since we assumed $a_i(t) > \epsilon $ over $t \in [0,T]$. Since furthermore $\left \lvert \Omega _{g,\bm X}(s)\right \rvert \le 1$, and since $N_{\bm X}(t) \in {0,1}$, the expectation is positive and bounded above by $$\epsilon ^{-2} \E {\int _{0}^t \partial N_{\bm X}(s)} = \epsilon ^{-2} \E {N_{\bm X}(t)} \le \epsilon ^{-2} < \infty .$$ \par Call now $$V_{g,h}(t) = \E {\Omega _{g,h}(\bm X) \int _{0}^t \frac {\partial N_{\bm X}(s)}{a_{\bm X}(s)^2}}.$$ \par Since $\bm \Gamma (t) = \left [\bm Z\right ](t)$ is by construction semi-definite positive, $\bm V(t)$ also is and \cref {itm:cv_Gamma} holds. \par \emph {Proof of \cref {itm:cv_Z}:} The Gaussian limit of $n^{-\frac {1}{2}}\bm Z$ comes directly from Robolledo's martingale central limit theorem, see \cite [Theorem II.5.1]{andersenCountingProcessModels1984}. There are two main conditions for this result to hold: \begin {itemize} \item $\forall t, \left [ \frac {\bm Z}{\sqrt {n}}\right ](t) \xrightarrow [n \to \infty ]{\mathbb P} \bm V(t)$, where $\bm V(t)$ is a deterministic function with semi-definite positive matrix values, \item $\forall t, \forall g\in G, \forall \eta > 0, \left \langle K_{g,\eta } \right \rangle (t) \xrightarrow [n \to \infty ]{\mathbb P} 0$, where $K_{g,\eta }$ is a martingale that contains all jumps of $\frac {Z_g}{\sqrt {n}}$ of size greater than $\eta $ \emph {(Lindeberg's condition).} \end {itemize} \par The first condition is exactly \cref {itm:cv_Gamma} we just proved. The remaining Lindeberg condition can be verified as follows. Let us first construct $K_{g,\eta }$ as the restriction of $\frac {Z_g}{\sqrt {n}}$ to jumps of size greater than $\eta $. For that, recall from \cref {eq:Z} that, under the null, \par \begin {align*} \frac {Z_g(t)}{\sqrt {n}} &= \int _{0}^t \frac {1}{\sqrt {n}}\sum _{\ell \in G} H_{g,\ell }(s)\partial \tld {M}_{E,\ell }(s)\\ &= \int _{0}^t \frac {1}{\sqrt {n}}\sum _{\ell \in G} H_{g,\ell }(s)\partial \sum _{i \in \ell } \frac {\partial M_i(s)}{a_i(s)}\\ &= \int _{0}^t \sum _{i =1}^n \frac {H_{g,\ell }(s)}{a_i(s)\sqrt {n}} \partial M_i(s) \end {align*} \par Then, since $N_i$'s have jumps of size 1, we can define the local square integrable martingale satisfying the requirement $K_{g,\eta }(t)$ as follows: $$K_{g,\eta }(t) = \sum _{i =1}^n \int _{0}^t \frac {H_{g,\ell }(s)}{a_i(s)\sqrt {n}} \I {\left \lvert \frac {H_{g,\ell }(s)}{a_i(s)\sqrt {n}} \right \rvert > \eta } \partial M_i(s).$$ \par \par Now, remembering that $\partial \langle M_i\rangle (s) = a_i(s)^2 \partial \Lambda _E(s)$, the predictable variate process of $K_{g,\eta }$ can be developed as: \begin {align} \left \langle K_{g,\eta }\right \rangle (t) &= \sum _{i =1}^n \int _{0}^t \left (\frac {H_{g,\ell }(s)}{a_i(s)\sqrt {n}}\right )^2 \I {\left \lvert \frac {H_{g,\ell }(s)}{a_i(s)\sqrt {n}} \right \rvert > \eta } \partial \langle M_i\rangle (s)\nonumber \\ &= \frac {1}{n}\sum _{i =1}^n \int _{0}^t H_{g,\ell }(s)^2 \I {\left \lvert H_{g,\ell }(s) \right \rvert > \eta \sqrt {n} a_i(s)}\partial \Lambda _E(s)\nonumber \\ &\le \frac {1}{n}\sum _{i =1}^n \int _{0}^t \I {\left \lvert H_{g,\ell }(s) \right \rvert > \eta \sqrt {n} a_i(s)} \partial \Lambda _E(s)\label {eq:uperbound}\\ &\xrightarrow [n \to \infty ]{\mathbb P} 0,\label {eq:cvtozero} \end {align} where the upper bound in \cref {eq:uperbound} is holding since $\lvert H_{g,\ell }(s) \rvert \le 1$. Moreover, as soon as $n \ge \eta ^{-2} a_i(s)^{-2} \ge \eta ^{-2}\epsilon ^{-2}$ (since we assumed $a_i(s) \ge \epsilon $ over $s \in [0,T]$), the indicatrix $$\I {\lvert H_{g,\ell }(s)\rvert > \epsilon \sqrt {n}a_i(s)}$$ is forced to be zero, and so the whole $\left \langle K_{g,\epsilon }\right \rangle (t)$ become zero after this particular $n$: the limit from \cref {eq:cvtozero} therefore holds and the Lindeberg's condition is fulfilled. \par \emph {Proof of \cref {itm:rank_V}:} We want to show that $\mathrm {Ker}(\bm V(t)) = \mathrm {Vect}(\bm 1)$. Recall the expressions for elements of $\bm V(t)$: $$V_{g,h}(t) = \E {\Omega _{g,h}(\bm X) \int _{0}^t \frac {\partial N_{\bm X}(s)}{a_{\bm X}(s)^2}}.$$ Remark that the matrix $\bm \Omega (\bm X)$ can only take $\lvert G \rvert $ different values, depending on the group assignment of $\bm X$. Consider then the vectorized notations: \begin {align*} g(\bm X) &= g \in G\text { s.t. }\bm X \in g\\ \bm i_g &= \left (\I {h =g}, h \in G\right )\\ \bm p &= \left (\P {\bm X \in g}, g \in G\right )\\ \bm \Omega _g &= \left (\bm i_g - \bm p\right )\left (\bm i_g - \bm p\right )', \end {align*} so that we can write the matrix $\bm \Omega (\bm X)$ as $\bm \Omega _{g(\bm X)}$. Now, $\forall \bm u \in \mathbb R^{\lvert G \rvert }$, \begin {align*} \bm u \in \mathrm {Ker}(\bm \Omega _g) &\iff \bm u'\Omega _g\bm u = 0\\ &\iff \bm u' \left (\bm i_g - \bm p\right )\left (\bm i_g - \bm p\right )' \bm u = 0\\ &\iff \lVert \bm u' \left (\bm i_g - \bm p\right ) \rVert _2^2 = 0\\ &\iff u_g = \bm u'\bm p \end {align*} Moreover, we can decompose $\bm V(t)$ as: \begin {align*} \bm V(t) &= \E {\Omega (\bm X) \int _{0}^t \frac {\partial N_{ \bm X}(s)}{a_{\bm X}(s)^2}}\\ &= \sum _{g \in G} \bm \Omega _g \E {\int _{0}^t \frac {\partial N_{ \bm X}(s)}{a_{\bm X}(s)^2}}{\bm X \in g} \P {\bm X \in g}\\ &= \sum _{g \in G} w_g \bm \Omega _g, \end {align*} Assuming without loss of generality that the probability of uncensored deaths occurring before time $t$ is strictly positive in each group, the weights $w_g$ are all strictly positives. Since moreover matrices $\Omega _g$ are all semi-definite positives, \begin {align*} \mathrm {Ker}(\bm V(t)) &= \bigcap _{g \in G} \mathrm {Ker}(\bm \Omega _g)\\ &= \bigcap _{g \in G} \{\bm u \in \mathbb R^{\lvert G \rvert }: \; u_g = \bm u'\bm p\}\\ &= \{\bm u \in \mathbb R^{\lvert G \rvert }: \forall g \in G \; u_g = \bm u'\bm p\}\\ &= \mathrm {Vect}(\bm 1). \end {align*}\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}This result is directly drawn from \cref {lem:test}, from which we fetched the condition on the coefficients, since \cref {lem:test} gives us that $$n^{-\frac {1}{2}}\bm Z(t) \xrightarrow [n\to \infty ]{\mathcal D} \N {0,\bm V(t)}.$$ From \cref {lem:test} again, we have $\mathrm {rank}(\bm V(t)) = \lvert G \rvert - 1$, the number of degree of freedom in the resulting $\chi ^2$ distribution is $\lvert G \rvert - 1$.\end{proof}

